Entropy on regular trees

We show that the limit in our definition of tree shift topological entropy is actually the infimum, as is the case for both the topological and measure-theoretic entropies in the classical situation when the time parameter is $\mathbb Z$. As a consequence, tree shift entropy becomes somewhat easier to work with. For example, the statement that the topological entropy of a tree shift defined by a one-dimensional subshift dominates the topological entropy of the latter can now be extended from shifts of finite type to arbitrary subshifts. Adapting to trees the strip method already used to approximate the hard square constant on $\mathbb Z^2$, we show that the entropy of the hard square tree shift on the regular $k$-tree increases with $k$, in contrast to the case of $\mathbb Z^k$. We prove that the strip entropy approximations increase strictly to the entropy of the golden mean tree shift for $k=2,\dots,8$ and propose that this holds for all $k \geq 2$. We study the dynamics of the map of the simplex that advances the vector of ratios of symbol counts as the width of the approximating strip is increased, providing a fairly complete description for the golden mean subshift on the $k$-tree for all $k$. This map provides an efficient numerical method for approximating the entropies of tree shifts defined by nearest neighbor restrictions. Finally, we show that counting configurations over certain other patterns besides the natural finite subtrees yields the same value of entropy for tree SFT's.

==> TreeShifts.ltb.tex <==
\bib{AB1}{article}{
   author={Aubrun, Nathalie},
   author={B\'eal, Marie-Pierre},
   title={Decidability of conjugacy of tree-shifts of finite type},
   conference={
      title={Automata, languages and programming. Part I},
   },
   book={
      series={Lecture Notes in Comput. Sci.},
      volume={5555},
      publisher={Springer, Berlin},
   },
   date={2009},
   pages={132--143},
   review={\MR{2544841}},
  % doi={10.1007/978-3-642-02927-1_13},
}
		
		\bib{AB2}{article}{
			author={Aubrun, Nathalie},
			author={B\'eal, Marie-Pierre},
			title={Sofic and almost of finite type tree-shifts},
			conference={
				title={Computer science---theory and applications},
			},
			book={
				series={Lecture Notes in Comput. Sci.},
				volume={6072},
				publisher={Springer, Berlin},
			},
			date={2010},
			pages={12--24},
			review={\MR{2972321}},
		%	doi={10.1007/978-3-642-13182-0_2},
		}
	
	\bib{AB3}{article}{
		author={Aubrun, Nathalie},
		author={B\'eal, Marie-Pierre},
		title={Tree-shifts of finite type},
		journal={Theoret. Comput. Sci.},
		volume={459},
		date={2012},
		pages={16--25},
		issn={0304-3975},
		review={\MR{2974235}},
		doi={10.1016/j.tcs.2012.07.020},
	}

\bib{AB4}{article}{
	author={Aubrun, Nathalie},
	author={B\'eal, Marie-Pierre},
	title={Sofic tree-shifts},
	journal={Theory Comput. Syst.},
	volume={53},
	date={2013},
	number={4},
	pages={621--644},
	issn={1432-4350},
	review={\MR{3084356}},
	doi={10.1007/s00224-013-9456-1},
}

\bib{AB5}{article}{
	author={Aubrun, Nathalie},
	author={B\'eal, Marie-Pierre},
	title={Tree algebra of sofic tree languages},
	journal={RAIRO Theor. Inform. Appl.},
	volume={48},
	date={2014},
	number={4},
	pages={431--451},
	issn={0988-3754},
	review={\MR{3302496}},
	doi={10.1051/ita/2014018},
}

\bib{BC1}{article}{
	author={Ban, Jung-Chao},
	author={Chang, Chih-Hung},
	title={Tree-shifts: Irreducibility, mixing, and the chaos of tree-shifts},
	journal={Trans. Amer. Math. Soc.},
	volume={369},
	date={2017},
	number={12},
	pages={8389--8407},
	issn={0002-9947},
	review={\MR{3710629}},
}


\bib{BC2}{article}{
	author={Ban, Jung-Chao},
	author={Chang, Chih-Hung},
	title={Mixing properties of tree-shifts},
	journal={J. Math. Phys.},
	volume={58},
	date={2017},
	number={11},
	pages={112702, 13},
	issn={0022-2488},
	review={\MR{3725174}},
}



\bib{BC3}{article}{
	author={Ban, Jung-Chao},
	author={Chang, Chih-Hung},
	title={Tree-shifts: {T}he entropy of tree-shifts of finite type},
	journal={Nonlinearity},
	volume={30},
	date={2017},
	number={7},
	pages={2785--2804},
	issn={0951-7715},
	review={\MR{3670007}},
}






\bib{BC4}{article}{
	author={Ban, Jung-Chao},
	author={Chang, Chih-Hung},
	title={Characterization for entropy of shifts of finite type on {C}ayley trees},
	eprint = {arXiv:1705.03138v1 [math.DS] 9 May 2017},
	date={2017},
}



\bib{BC5}{article}{
	author={Ban, Jung-Chao},
	author={Chang, Chih-Hung},
	author={Huang, Nai-Zhu},
	title={Entropy bifurcation of neural networks on {C}ayley trees},
	eprint = {arXiv:1706.09283v1 [math.DS] 27 Jun 2017},
	date={2017},
}

\bib{BC6}{article}{
	author={Ban, Jung-Chao},
	author={Chang, Chih-Hung},
	title={Coloring {F}ibonacci-{C}ayley tree: {A}n application to neural networks},
	eprint = {arXiv:1707.02227v1 [math.DS] 5 Jul 2017},
	date={2017},
}

\bib{BP1994}{article}{
	author={Benjamini, Itai},
	author={Peres, Yuval},
	title={Markov chains indexed by trees},
	journal={Ann. Probab.},
	volume={22},
	date={1994},
	number={1},
	pages={219--243},
	issn={0091-1798},
	review={\MR{1258875}},
}

\bib{Berstel2010}{article}{
	author={Berstel, Jean},
	author={Boasson, Luc},
	author={Carton, Olivier},
	author={Fagnot, Isabelle},
	title={Sturmian trees},
	journal={Theory Comput. Syst.},
	volume={46},
	date={2010},
	number={3},
	pages={443--478},
	issn={1432-4350},
	review={\MR{2592178}},
}

\bib{Bowen 2017}{article}{
	author={Bowen, Lewis},
	title={A brief inytroduction to sofic entropy theory},
	eprint = {arXiv:1711.02062v1 [math.DS] 6 Nov 2017},
	date={2017},
}

\bib{BPS1995}{article}{
	author={Burton, R. M.},
	author={Pfister, C.-E.},
	author={Steif, J. E.},
	title={The variational principle for Gibbs states fails on trees},
	journal={Markov Process. Related Fields},
	volume={1},
	date={1995},
	number={3},
	pages={387--406},
	issn={1024-2953},
	review={\MR{1403088}},
}

\bib{Carpi2001}{article}{
	author={Carpi, A.},
	author={de Luca, A.},
	author={Varricchio, S.},
	title={Special factors and uniqueness conditions in rational trees},
	journal={Theory Comput. Syst.},
	volume={34},
	date={2001},
	number={4},
	pages={375--395},
	issn={1432-4350},
	review={\MR{1845664}},
}

\bib{CP}{article}{
	author={Carroll, Kathleen},
	author={Petersen, Karl},
	title={Markov diagrams for some non-Markovian systems},
	conference={
		title={Ergodic {T}heory, {D}ynamical {S}ystems, and the {C}continuing {I}nfluence
			of John C. Oxtoby},
	},
	book={
		series={Contemp. Math.},
		volume={678},
		publisher={Amer. Math. Soc., Providence, RI},
	},
	date={2016},
	pages={73--101},
	review={\MR{3589817}},
}

\bib{CovenHedlund1973}{article}{
	author={Coven, Ethan M.},
	author={Hedlund, G. A.},
	title={Sequences with minimal block growth},
	journal={Math. Systems Theory},
	volume={7},
	date={1973},
	pages={138--153},
	issn={0025-5661},
	review={\MR{0322838}},
}

\bib{Cyr-Kra}{article}{
	author={Cyr, Van},
	author={Kra, Bryna},
	title={Nonexpansive $\Bbb{Z}^2$-subdynamics and Nivat's conjecture},
	journal={Trans. Amer. Math. Soc.},
	volume={367},
	date={2015},
	number={9},
	pages={6487--6537},
	issn={0002-9947},
	review={\MR{3356945}},
}

\bib{Epifanio}{article}{
	author={Epifanio, Chiara},
	author={Koskas, Michel},
	author={Mignosi, Filippo},
	title={On a conjecture on bidimensional words},
	journal={Theoret. Comput. Sci.},
	volume={299},
	date={2003},
	number={1-3},
	pages={123--150},
	issn={0304-3975},
	review={\MR{1973149}},
}

\bib{GamarnikKatz2009}{article}{
	author={Gamarnik, David},
	author={Katz, Dmitriy},
	title={Sequential cavity method for computing free energy and surface
		pressure},
	journal={J. Stat. Phys.},
	volume={137},
	date={2009},
	number={2},
	pages={205--232},
	issn={0022-4715},
	review={\MR{2559429}},
	doi={10.1007/s10955-009-9849-3},
}

\bib{GastGaujal2010}{article}{
	author={Gast, Nicolas},
	author={Gaujal, Bruno},
	title={Infinite labeled trees: from rational to Sturmian trees},
	journal={Theoret. Comput. Sci.},
	volume={411},
	date={2010},
	number={7-9},
	pages={1146--1166},
	issn={0304-3975},
	review={\MR{2606051}},
	doi={10.1016/j.tcs.2009.12.009},
}


\bib{Georgii}{book}{
	author={Georgii, Hans-Otto},
	title={Gibbs {M}easures and {P}hase {T}ransitions},
	series={De Gruyter Studies in Mathematics},
	volume={9},
	edition={2},
	publisher={Walter de Gruyter \& Co., Berlin},
	date={2011},
	pages={xiv+545},
	isbn={978-3-11-025029-9},
	review={\MR{2807681}},
	doi={10.1515/9783110250329},
}


\bib{HM}{article}{
	author={Morse, Marston},
	author={Hedlund, Gustav A.},
	title={Symbolic dynamics},
	journal={Amer. J. Math.},
	volume={60},
	date={1938},
	number={4},
	pages={815--866},
	issn={0002-9327},
	review={\MR{1507944}},
}

\bib{HochmanMeyerovitch2010}{article}{
	author={Hochman, Michael},
	author={Meyerovitch, Tom},
	title={A characterization of the entropies of multidimensional shifts of
		finite type},
	journal={Ann. of Math. (2)},
	volume={171},
	date={2010},
	number={3},
	pages={2011--2038},
	issn={0003-486X},
	review={\MR{2680402}},
	doi={10.4007/annals.2010.171.2011},
}

\bib{KerrLi2016}{book}{
	author={Kerr, David},
	author={Li, Hanfeng},
	title={Ergodic {T}heory},
	series={Springer Monographs in Mathematics},
	note={Independence and dichotomies},
	publisher={Springer, Cham},
	date={2016},
	pages={xxxiv+431},
	isbn={978-3-319-49845-4},
	isbn={978-3-319-49847-8},
	review={\MR{3616077}},
	doi={10.1007/978-3-319-49847-8},
}

\bib{KimLim2015}{article}{
	author={Kim, Dong Han},
	author={Lim, Seonhee},
	title={Subword complexity and Sturmian colorings of regular trees},
	journal={Ergodic Theory Dynam. Systems},
	volume={35},
	date={2015},
	number={2},
	pages={461--481},
	issn={0143-3857},
	review={\MR{3316921}},
	doi={10.1017/etds.2013.50},
}

\bib{LM}{book}{
	author={Lind, Douglas},
	author={Marcus, Brian},
	title={An {I}ntroduction to {S}ymbolic {D}ynamics and {C}oding},
	publisher={Cambridge University Press, Cambridge},
	date={1995},
	pages={xvi+495},
	isbn={0-521-55124-2},
	isbn={0-521-55900-6},
	review={\MR{1369092}},
}

\bib{LouidorMarcusPavlov2013}{article}{
	author={Louidor, Erez},
	author={Marcus, Brian},
	author={Pavlov, Ronnie},
	title={Independence entropy of $\Bbb{Z}^d$-shift spaces},
	journal={Acta Appl. Math.},
	volume={126},
	date={2013},
	pages={297--317},
	issn={0167-8019},
	review={\MR{3077954}},
	doi={10.1007/s10440-013-9819-2},
}

\bib{MairesseMarcovici2017}{article}{
	author={Mairesse, Jean},
	author={Marcovici, Ir\`ene},
	title={Uniform sampling of subshifts of finite type on grids and trees},
	journal={Internat. J. Found. Comput. Sci.},
	volume={28},
	date={2017},
	number={3},
	pages={263--287},
	issn={0129-0541},
	review={\MR{3652917}},
	doi={10.1142/S0129054117500174},
}

\bib{MarcusPavlov2013}{article}{
	author={Marcus, Brian},
	author={Pavlov, Ronnie},
	title={Approximating entropy for a class of $\Bbb Z^2$ Markov random
		fields and pressure for a class of functions on $\Bbb Z^2$ shifts of
		finite type},
	journal={Ergodic Theory Dynam. Systems},
	volume={33},
	date={2013},
	number={1},
	pages={186--220},
	issn={0143-3857},
	review={\MR{3009110}},
	doi={10.1017/S0143385711000824},
}

\bib{MeyerovitchPavlov2014}{article}{
	author={Meyerovitch, Tom},
	author={Pavlov, Ronnie},
	title={On independence and entropy for high-dimensional isotropic
		subshifts},
	journal={Proc. Lond. Math. Soc. (3)},
	volume={109},
	date={2014},
	number={4},
	pages={921--945},
	issn={0024-6115},
	review={\MR{3273488}},
	doi={10.1112/plms/pdu029},
}
 
\bib{OEIS}{webpage}{
	title = {The Online Encyclopedia of Integer Sequences},
	url = {https://oeis.org},
}

\bib{Pavlov2012}{article}{
	author={Pavlov, Ronnie},
	title={Approximating the hard square entropy constant with probabilistic
		methods},
	journal={Ann. Probab.},
	volume={40},
	date={2012},
	number={6},
	pages={2362--2399},
	issn={0091-1798},
	review={\MR{3050506}},
	doi={10.1214/11-AOP681},
}

\bib{KPSalta}{webpage}{
	title = {Measuring {C}omplexity in {C}antor {D}ynamics},
		author={Karl Petersen},
	url = {http://www.unc.edu/math/Faculty/petersen/Papers/KEPSalta2016_07_08.pdf},
}

\bib{PS2018}{article}{
author={Petersen, Karl},
author={Salama, Ibrahim},
title={Tree shift topological entropy},
journal={Theoretical Computer Science},
date={6 June 2018},
note={DOI: 10.1016/j.tcs.2018.05.034},
url={https://doi.org/10.1016/j.tcs.2018.05.034},	
}

\bib{Piantadosi2008}{article}{
	author={Piantadosi, Steven T.},
	title={Symbolic dynamics on free groups},
	journal={Discrete Contin. Dyn. Syst.},
	volume={20},
	date={2008},
	number={3},
	pages={725--738},
	issn={1078-0947},
	review={\MR{2373212}},
	doi={10.3934/dcds.2008.20.725},
}

\bib{Preston1974}{book}{
	author={Preston, Christopher J.},
	title={Gibbs {S}tates on {C}ountable {S}ets},
	note={Cambridge Tracts in Mathematics, No. 68},
	publisher={Cambridge University Press, London-New York},
	date={1974},
	pages={ix+128},
	review={\MR{0474556}},
}


\bib{Spitzer1975}{article}{
	author={Spitzer, Frank},
	title={Markov random fields on an infinite tree},
	journal={Ann. Probability},
	volume={3},
	date={1975},
	number={3},
	pages={387--398},
	review={\MR{0378152}},
}
